Beyond Generating Code: Evaluating GPT on a Data Visualization Course

This paper presents an empirical evaluation of the performance of the Generative Pre-trained Transformer (GPT) model in Harvard's CS171 data visualization course. While previous studies have focused on GPT's ability to generate code for visualizations, this study goes beyond code generation to evaluate GPT's abilities in various visualization tasks, such as data interpretation, visualization design, visual data exploration, and insight communication. The evaluation utilized GPT-3.5 and GPT-4 to complete assignments of CS171, and included a quantitative assessment based on the established course rubrics, a qualitative analysis informed by the feedback of three experienced graders, and an exploratory study of GPT's capabilities in completing border visualization tasks. Findings show that GPT-4 scored 80% on quizzes and homework, and TFs could distinguish between GPT- and human-generated homework with 70% accuracy. The study also demonstrates GPT's potential in completing various visualization tasks, such as data cleanup, interaction with visualizations, and insight communication. The paper concludes by discussing the strengths and limitations of GPT in data visualization, potential avenues for incorporating GPT in broader visualization tasks, and the need to redesign visualization education.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> tex/_deprecated/3-exp.tex <==
\section{GPT for CS171 - a Data Visualization Course}

This section will first introduce Harvard's undergraduate visualization course CS171
and then outline the settings of our experiments.

\subsection{CS171 at Harvard}
% CS171 is an introductory course that teaches students key design principles and techniques for interactively visualizing data. 
% %% learning objectives
% The course is designed to help students
% understand the fundamental concepts and principles of data visualization and visual analytics. 
% It covers topics on how to design, create, critique, and refine visualizations. 
% It also teaches students how to 
% create web-based interactive visualizations using Javascript and D3, and how to conceptualize ideas and interaction techniques using sketching and prototyping.
% Finally, it teaches students how to
% apply visualization methods to display data from a variety of fields, 
% and how to work constructively as a team member to carry out a visualization project.

CS171 is an introductory course at Harvard for data visualization. The course covers key design principles, design processes, and web-based programming skills for data visualization. 
% After taking the course, students will receive a letter grade, 
% ranging from A (95-100\%) to F ($<$45\%), with several components contributing to the final grade: 
Students' grades will be determined based on their participation in class activities (accounts for 10\%) and their performance on the following tasks:

    % \begin{figure}[h]
    %     \centering
    %     \includegraphics[width=0.9\linewidth]{figures/quiz_exp.jpg}
    %     \vspace{-2mm}
    %     \caption{A quiz example.}
    %     \vspace{-2mm}
    %     \label{fig:quiz_exp}
    % \end{figure}

    % \item \emph{Quizzes (25\%)} are designed to evaluate students' 
    % understanding of visualization design principles
    % and web programming,
    % and their ability to apply them to specific scenarios. 
    % A quiz can include several single-choice, multiple-choice, or matching questions.
    % Each question has a ground truth answer and thus can be graded automatically.

    \para{Quizzes (25\%)} are a set of objective questions, including single-choice, multiple-choice, and matching questions.
    These questions cover a range of visualization knowledge, including design principles, web programming, and practical applications. CS171 contains 91 quiz questions.
    % Figure~\ref{fig:quiz_exp} shows an example of a single-choice question in a quiz.
    % \cmo{a statistic of the quizzes.}

    % \begin{figure}[h]
    %     \centering
    %     \includegraphics[width=1\linewidth]{figures/hw_exp.jpg}
    %     \vspace{-2mm}
    %     \caption{An example of the instructions in a programming homework.}
    %     \vspace{-2mm}
    %     \label{fig:hw_exp}
    % \end{figure}

    % \item \emph{Programming Homework (30\%)} requires students to apply the concepts learned in class and labs. 
    % These assignments test the students' coding skills and understanding of how to create interactive visualizations using JavaScript and D3. 
    % Each assignment consists of several tasks, given datasets, step-by-step instructions, or code templates to help students finish the programming tasks.
    % Some tasks also ask students to write essays on the pros and cons of given visualizations or to redesign them.
    % Figure~\ref{fig:hw_exp} displays an example of an assignment.
    % Each assignment is graded by teaching assistants based on a rubric.
    % In total, there are nine assignments (Week 1 - Week 9) in CS171.

    \para{Homeworks (30\%)} are subjective questions requiring students to write essays and (or) code for visualization design, evaluation, and implementation. Each assignment includes tasks, datasets, instructions, and code templates. Teaching fellows grade assignments using rubrics. CS171 includes nine assignments spanning nine weeks.

    \para{Final Project (35\%)} requires students to work in teams of three to design and implement an interactive storytelling website on a topic of their choice.
    The final project is graded based on the quality of the visualizations, 
    the effectiveness of the data storytelling, 
    and the creativity and innovation of the design.


% Additionally, class activities also contribute 10\% towards the grade. \jb{add the percentage of how quizzes, hw, and the final project contribute}


\subsection{Evaluating GPT on CS171}
% \cmo{need to say G3 vs G4}

% Our objective is to evaluate whether GPT can perform as a student in CS171.
% % and how effectively it can complete the course components
% To accomplish this, 
% we decided to have GPT complete the assignments from CS171 directly, 
% rather than using GPT as a tool to aid a human in completing assignments.
Two GPT models, GPT3.5 and GPT4, are evaluated on the course components. 
To accurately assess the inherent capabilities of GPT models, we conduct a zero-shot evaluation without employing complex prompting strategies or domain-specific fine-tuning.
Specifically, we design our experiments as follows:

\para{Quizzes.}
The prompt template for quizzes is shown below. 
The \texttt{question type} indicates whether it is a single-choice, multi-choice, or matching question.
The \texttt{format requirements} is decided based on the question type.
We repeat each question 10 times and calculate the average grade.

\begin{coloredquotation}
    \textbf{Prompt template for quiz:}\\
    The following is a quiz question, please give your answer in the following format \{ \texttt{format requirements} \}.\\
    \{ \texttt{question type} \} \\
    \{ \texttt{quiz question} \}
\end{coloredquotation}


% The answers are then automatically graded against the correct answers.


\para{Homework.}
% \cmo{a figure to demonstrate the prompt here might be helpful}
% We ask GPT to finish the programming homework solely based on the assignment instructions.
% Due to the token length restriction,
% we provide GPT with one step of the instruction at a time.
% File content of the templates in the instructions was supplied when necessary.
% We use minimal prompts to ensure GPT outputs the code directly,
% such as \emph{``print the code you changed in main.js''}

The prompt template for homework is shown below. 
To accommodate the token length limitation, GPT receives each step sequentially from the step-by-step instructions.
When necessary, the content of file templates referenced in the instructions is provided.

\begin{coloredquotation}
    \textbf{Prompt template for homework:}\\
    \{  \texttt{one step of the introductions} \} \\
    \{ \texttt{content of the related template file} \} \\
    Please output the changes you made to \{\texttt{name of the template file}  \}
\end{coloredquotation}

We added the code generated by GPT into template files and execute them in a browser. 
If an error arises, we re-generate the response; otherwise, we move forward to the next instruction.

\cmo{@zhutian, what is the upper limit that you will stop regenerating and say the GPT fails??}

%% grading
For the grading process, three CS171 TFs, who are also coauthors, independently assess the assignments using a long-established rubric that has been employed in the course for many years. 
To prevent bias, assignments from GPT are mixed with past student submissions, and the three graders are unaware of their origin. 
Each assignment is graded by two teaching fellows, and the scores are then averaged.
After grading an assignment, a TF assessed whether the assignment is generated by human or AI using a 5-point likert scale, 1 indicate ``definitely human'' and 5 indicates ``definitely AI''. TFs also offered free-form comments that addressed various aspects of the assignment, including the structure of the code, the quality of the documentation, and the creativity demonstrated in the work.
% To avoid bias toward machine or human work,
% we mixed these assignments with past students' submissions
% and assign each TA two assignments for each week's homework, 
% each of which may be completed by either GPT or a student.
% The TAs were not informed of whether the assignments were completed by GPT or students. Furthermore, each machine assignment is graded by two TAs, and their scores are averaged.


\para{Final Project.}
% We chose not to ask GPT to complete the final project as it is a group project graded on teamwork and peer evaluation. Instead, we used the CS171 final project guidelines as a checklist to qualitatively assess GPT's ability to support the completion of a final project, including data collection, data cleanup,
% data analysis with exploratory visualizations, 
% data insights communication with explainatory visualizations.
% Our aim was to determine whether GPT possesses the fundamental capabilities required to complete a typical visualization project. 
% Our exploration was open-ended and intended to serve as a reference for inspiring future research.
We did not directly evaluate GPTs on the final project due to its team-based nature and its reliance on peer evaluation.
Instead,
we evaluate GPTs at each step of a visualization project, including data collection, data cleanup, task summarization, visualization design, visual exploration, and insight communication.
\cmo{if possible, provide a citation for these steps here}.
We present examples and share insights into GPT's capabilities and limitations at each step of the process.
% We hope these open-ended explorations can help inspire future research.

\cmo{[Qianwen:] @Zhutian, can you provide a prompt template here for these open-ended explorations}

% We prompt GPT with the final project's descriptions, asking GPT to generate a detailed project plan with steps.
% Then, we prompt GPT to finish its plan step by step.
% We also use these steps to guide us explore GPT's capabilities in a broader 
% We decided not to grade the final project but only qualitatively probe into GPT's capabilities in finishing the project.


==> tex/_deprecated/4-result_v1.tex <==
\section{Results}

\setlength{\tabcolsep}{1pt}
\begin{table}[h]
    \centering
    \small
    % \vspace{-2mm}
    \caption{GPTs' scores on the Quizzes and Homework.\jb{can you show percentages instead of scores? scores make no sense if I don't know the maximum score}}
    \label{table:scenes}
    % \vspace{-2mm}
    \begin{tabular}{l|
    >{\centering\arraybackslash}p{8mm}
    >{\centering\arraybackslash}p{10mm}|
    >{\centering\arraybackslash}p{4mm}
    >{\centering\arraybackslash}p{4mm}
    >{\centering\arraybackslash}p{4mm}
    >{\centering\arraybackslash}p{4mm}
    >{\centering\arraybackslash}p{4mm}
    >{\centering\arraybackslash}p{4mm}
    >{\centering\arraybackslash}p{4mm}
    >{\centering\arraybackslash}p{4mm}
    >{\centering\arraybackslash}p{4mm}|
    >{\centering\arraybackslash}p{14mm} 
}
    \toprule
      % & Quizzes & Homework & \\ \midrule
      % & Quizzes & Homework & \\ \midrule

     & \multicolumn{2}{c|}{\textbf{Quizzes}} & \multicolumn{9}{c|}{\textbf{Homework}} & \textbf{Weight Sum} \\ 
     & Pre-lab & Post-class & \MYhref{https://www.cs171.org/Homework_instructions/week-01/week_01_hw.html}{W1} & 
     \MYhref{https://www.cs171.org/Homework_instructions/week-02/hw/HW2.html}{W2} & 
     \MYhref{https://www.cs171.org/Homework_instructions/week-03/hw/week-03_hw.html}{W3} & 
     \MYhref{https://www.cs171.org/Homework_instructions/week-04/hw/week-04_hw.html}{W4} &
     \MYhref{https://www.cs171.org/Homework_instructions/week-05/hw/week_05_hw.html}{W5} &
     \MYhref{https://www.cs171.org/Homework_instructions/week-06/hw/week-06_hw.html}{W6} & 
     \MYhref{https://www.cs171.org/Homework_instructions/week-07-design/week-07_design.html}{W7} & 
     \MYhref{https://www.cs171.org/Homework_instructions/week-08/hw/week-08_hw.html}{W8} & 
     \MYhref{https://www.cs171.org/Homework_instructions/week-09/hw/week-09_hw.html}{W9} & (\%) \\ \midrule
    \textbf{GPT-3.5} & 4.3 & 30.03 & 8 & 7.5 & 8.8 & 9.5 & 11 & 10 & 4 & 9.3 & 1 &   39.8 (72.3\%) \\
    \textbf{GPT-4} & 5.03 & 39.82 & 8 & 9.5  & 6.3 & 10 & 9.5 & 7.3 & 5.3 & 9 & 8 & 
    \textbf{45.5 (82.7\%)} \\ 
    \bottomrule
    \end{tabular}
 	% \vspace{-2mm}
\end{table}


\subsection{Quiz}

Both GPT-3.5 and GPT-4 completed most of the quizzes.
GPT-3.5 scored 68.8\% while GPT-4 scored 86.4\%.
These results overall indicate that GPT has a wide range of visualization knowledge, 
including design principles, web programming, and practical applications.
Below we discuss the failure cases of GPT in finishing the quizzes:

\begin{itemize}[leftmargin=*]
\item \textbf{GPT cannot read figures.}
Since the GPTs we utilized were incapable of taking images as input, 
they did not perform well on questions that required extracting information from images. 
Nevertheless, we are optimistic that a multi-modal GPT (such as the full version of GPT-4) will excel in these types of questions in the near future.

\item \textbf{Bad at matching questions.}
We discovered that GPTs did not excel in matching questions 
(e.g., \cmo{Need an example, @chenyang} \chenyang{ @zhutian, here are some examples (you can view in the Editor view because I comment them out ↓)}). 

% ```Example 1
% # assignment_Week 9 | HW Part 2 (Post-Lecture Quiz) | Question 3

% GPT Model: gpt-4

% Question type: matching_question

% Question:
% <div><p>Put the elements of the story narrative or story arc by Gustav Freytag in the correct order.</p></div>

% Choices:
% [[response_8920]] - 1.: [[5848]] - Exposition, [[2599]] - Raising Action, [[3213]] - Climax, [[2237]] - Falling Action, [[7652]] - Resolution
% [[response_7790]] - 2.: [[5848]] - Exposition, [[2599]] - Raising Action, [[3213]] - Climax, [[2237]] - Falling Action, [[7652]] - Resolution
% [[response_6881]] - 3.: [[5848]] - Exposition, [[2599]] - Raising Action, [[3213]] - Climax, [[2237]] - Falling Action, [[7652]] - Resolution
% [[response_8250]] - 4.: [[5848]] - Exposition, [[2599]] - Raising Action, [[3213]] - Climax, [[2237]] - Falling Action, [[7652]] - Resolution
% [[response_419]] - 5.: [[5848]] - Exposition, [[2599]] - Raising Action, [[3213]] - Climax, [[2237]] - Falling Action, [[7652]] - Resolution

% Correct Answers:
% [[response_8920]] - 1.: [[5848]] - Exposition
% [[response_7790]] - 2.: [[2599]] - Raising Action
% [[response_6881]] - 3.: [[3213]] - Climax
% [[response_8250]] - 4.: [[2237]] - Falling Action
% [[response_419]] - 5.: [[7652]] - Resolution

% ****************************************

% ATTEMPT 1

% Answer: 
% [[response_8920]] - 1.: [[5848]] - Exposition, [[2599]] - Raising Action, [[3213]] - Climax, [[2237]] - Falling Action, [[7652]] - Resolution

% Score: 0.0
% ```

% ===================================================
% ===================================================
% ===================================================

% ```Example 2
% # assignment_Week 9 | HW Part 2 (Post-Lecture Quiz) | Question 2

% GPT Model: gpt-4

% Question type: matching_question

% Question:
% <div><p>Assign the correct attributes to each term.</p></div>

% Choices:
% [[response_5052]] - Text is (pick 1-word answer): [[190]] - learned, [[2526]] - processed in parallel, [[9113]] - rational and abstract, [[6682]] - innate
% [[response_444]] - Visual information is (pick 3-word answer): [[190]] - learned, [[2526]] - processed in parallel, [[9113]] - rational and abstract, [[6682]] - innate
% [[response_2430]] - Text is (pick 3-word answer): [[190]] - learned, [[2526]] - processed in parallel, [[9113]] - rational and abstract, [[6682]] - innate
% [[response_6556]] - Visual information is (pick 1-word answer): [[190]] - learned, [[2526]] - processed in parallel, [[9113]] - rational and abstract, [[6682]] - innate

% Correct Answers:
% [[response_5052]] - Text is (pick 1-word answer): [[190]] - learned
% [[response_444]] - Visual information is (pick 3-word answer): [[2526]] - processed in parallel
% [[response_2430]] - Text is (pick 3-word answer): [[9113]] - rational and abstract
% [[response_6556]] - Visual information is (pick 1-word answer): [[6682]] - innate

% ****************************************

% ATTEMPT 1

% Answer: 
% [[response_5052]] - Text is (pick 1-word answer): [[9113]] - rational and abstract
% [[response_444]] - Visual information is (pick 3-word answer): [[2526]] - processed in parallel, [[190]] - learned, [[6682]] - innate
% [[response_2430]] - Text is (pick 3-word answer): [[9113]] - rational and abstract, [[190]] - learned, [[2526]] - processed in parallel
% [[response_6556]] - Visual information is (pick 1-word answer): [[2526]] - processed in parallel

% Score: 0.0
% ```

% ===================================================
% ===================================================
% ===================================================

% ```Example 3
% # assignment_Week 2 | HW Part 2 (Post-Lecture Quiz) | Question 5

% GPT Model: gpt-4

% Question type: matching_question

% Question:
% <div><p>Fill in the blanks:</p></div>

% Choices:
% [[response_8200]] - By default, Tableau Desktop aggregates: [[3372]] - measures, [[7208]] - dimension
% [[response_85]] - but does not aggregate: [[3372]] - measures, [[7208]] - dimension

% Correct Answers:
% [[response_8200]] - By default, Tableau Desktop aggregates: [[3372]] - measures
% [[response_85]] - but does not aggregate: [[7208]] - dimension

% ****************************************

% ATTEMPT 1

% Answer: 
% [[response_8200]] - By default, Tableau Desktop aggregates: [[3372]] - measures, [[7208]] - dimension
% [[response_85]] - but does not aggregate: [[7208]] - dimension

% Score: 0.5
% ```


We suspect that the text descriptions provided in these questions are too ambiguous for GPTs to comprehend and solve. 
However, humans can discern the intention of the questions from the user interfaces (i.e., the drop-down list). 
We believe that if a future version of GPT is capable of reading user interfaces, its performance in these tasks will be enhanced.

\end{itemize}

\subsection{Homework}

Both GPT-3.5 and GPT-4 were able to complete most of the homework assignments, with GPT-3.5 achieving a score of 22.6\% and GPT-4 achieving a score of 23.9\%. \jb{that is super low, is that out of 100 percent? (it should be)}
An example of the visualizations created by GPT-4 is shown in \autoref{fig:xx}. 
In the following section, we will discuss our observations and the feedback we received from the TFs.

\subsubsection{Observations in Using GPTs}
GPT clearly showed the capability to understand instructions and complete assignments. 
Through these assignments, 
GPT demonstrated knowledge of visualization theory (e.g., exploratory vs. explanatory visualizations, Gestalt principles), 
visualization design (e.g., design critiques),
web programming skills (e.g., HTML/CSS/JS),
data transformations,
and visualization-dedicated libraries (e.g., D3).
GPT-4 outperformed GPT-3.5 in many ways.
For example,
while GPT-3.5 typically needed dozens of attempts to develop one error-free solution, 
GPT-4 could come up with the correct solution in less than 10 retries.

Below we summarize the challenges we faced when using GPTs to finish CS171 homework assignments.
\begin{itemize}[leftmargin=*]
    \item \textbf{Versioning of programming libraries.}
    % GPTs struggled in using external libraries when different versions.
    For example, 
    when tasked to finish a programming task,
    GPT could refer to D3 version 7 in the HTML file but use the APIs from D3 version 6 in the JS file.
    This implies that GPT cannot reason about the relationship between the code files it generates.
    However, when the instructions explicitly mention the version of the libraries used, GPT can correctly generate the code.
    % Therefore, it is easy for the students to prompt GPT with the versions of the library.
    \qianwen{this example is confusing. I am not sure whether the problem is because that 1) GPT cannot understand library versions or 2) GPT can not associate different programming files. I feel like is more like 2) but you summarized it as 1). }
    
    \item \textbf{Outdated Knowledge.}
    Since GPT is trained on data collected before September 2021, it may generate outdated information.
    For example, HW1 asks for examples of good and bad visualizations and explanations of why they are good or bad. 
    % GPT will generate links to the visualizations and explanations.
    While the GPT generated reasonable explanations,
    the URL links to the visualizations were expired.
    % This is not surprise as GPT is trained on a dataset collected before 2021.
    
    \item \textbf{Hallucination.} The GPT versions we used do not support images as input. Thus, for assignments that contained images in their instructions, we simply provided a URL of the image.
    For example, in the assignment Week 2, GPT is asked to criticize a visualization of the top 10 salaries at Google. 
    Instead of acknowledging that it cannot read the image, GPT will ``imagine'' a visualization and discuss the pros and cons of it.
    This is the so-called ``hallucination'' phenomenon of GPT.
    \sw{Can we say more? Like this "hallucination" is bad, but i think it's important to emphasize that it made  references to things in the image that weren't real, or cite actual performance on these tasks}
    
    \item \textbf{Ethical Constraints.} Moderation layers have been introduced to GPTs to prevent content that violates OpenAI's usage policies. From time to time, GPT will respond that it cannot generate the code or answers for us since it is unethical to cheat in doing homework.
    \qianwen{@zhutian, can you add the exact output from GPT here}
    Nevertheless, this can simply be resolved by re-trying a few more times.
    
    %% failure
    \item{\textbf{Token Length Limitation.}}
    GPT has a limit on the token length (i.e., 4k for GPT-3.5, and 8k GPT-4). Thus, we sometimes could not input all the instructions, datasets, and code templates into GPT at once and had to break them into small chunks.
    However, the tasks in Week 9 still involved too many lines of code and could not meet the code line limit, even when breaking the tasks into smaller pieces.
    Thus, GPT-3.5 could not finish the assignment for Week 9.
    
\end{itemize}

%% struggle
% GPTs struggled in using external libraries.
% For example, 
% when asking GPT to finish a programming task by generating an HTML and JS file,
% it could refer to D3V7 in the HTML file but use the APIs from D3V6 in the JS.
% This implies that GPT cannot reasoning the relationship between the code files it generates.
% However, when the instruction explicitly mentions the version of the libraries used, GPT can correctly generate the codes.
% Therefore, it is easy for the students to prompt GPT with the versions of the library.

% \cmo{archive knowledge.}
% The assignment of Week1 asks GPT to provide examples of good and bad visualizations and explain why they are good or bad. 
% GPT will generate links to the visualizations and explanations.
% While the explanations read make sense,
% the links generally point to pages that do not exist.
% This is not surprise as GPT is trained on a dataset collected before 2021.

% \cmo{Hallucination.} The GPT version we used cannot take images as input. Thus, for some assignments that need to read images, we simply provide a URL of the image.
% For example, in the assignment Week2, GPT is asked to criticize a visualization of the top 10 salaries at Google. 
% Instead of acknowledging that it cannot read the image, GPT will ``imagine'' a visualization and discuss the pros and cons of it.
% This is the so-called ``hallucination'' phenomenon of GPT.

% \cmo{Ethics.} From time to time, GPT will respond that it cannot generate the codes or answers for us since it is unethical to cheat in doing homework.
% Nevertheless, this can simply be resolved by re-try a few more times.

% %% failure
% \cmo{Token Length.}
% GPT has a limit on the token length (i.e., GPT-3.5 for 4K and GPT-4 for 8K), and thus sometimes we cannot input all the instructions, datasets, and code templates into GPT and have to break them into small chunks.
% Nonetheless, the tasks in Week 9 involve too many codes and cannot meet the code limits even if we break them into small pieces.
% Thus, GPT-3.5 cannot finish the assignment for Week 9.

% \subsubsection{Feedback from TFs.}
\subsubsection{Feedback from Grading GPTs}
% \cmo{@Qianwen}
Overall, TFs were impressed by the quality of the GPT-generated homework assignments, which is also reflected by the grades (GPT-3.5 scored 75.2\% and GPT-4 scored 79.7\%).

TFs were able to accurately identify \textit{definitely GPT} or \textit{definitely human} HWs, but experienced uncertainty with assignments that fell in between, describing these HWs as \textit{``either a really bored student or an ok AI''} (TF2).
Among the total of 54 graded assessments (3 TFs $\times$ 9 HWs $\times$ 2 submissions per TF per HW), 
TFs had an impressive 100\% accuracy when they categorized the HWs as \textit{``definitely human''} (8 times), \textit{``definitely GPT''} (12 times), and \textit{``maybe GPT''} (14 times).
Such a high accuracy contrasts with the findings of previous research that evaluated humans' ability to distinguish GPT-generated texts from human-written texts in general tasks~\cite{jakesch2023human, clark2021all}, where humans showed similar accuracy as random guessing.
We hypothesize that this discrepancy in accuracy may be attributed to the distinctions between professional and non-professional contexts and the inherent differences between natural language text and programming code.
At the same time, GPT demonstrated a notable capacity to mislead the TFs to some degree.
When TFs categorized the HWs as \textit{``maybe human''}, the accuracy was only 33.3\% (4 correct identifications out of 12). In other words, on 8 out of the 12 occasions when TFs classified the homework assignments as \textit{``maybe human''}, the assignments were, in reality, generated by GPT.


The three TFs reported the heuristics they used to distinguish between assignments submitted by students and those generated by GPT. 
While these heuristics reveal valuable insights about GPT-generated assignments, they were not consistently true.
\begin{itemize}[leftmargin=*]
    \item \textbf{GPT lacks creativity [true].} TFs were able to identify student submissions based on the belief that \textit{``this level of creativity is not exhibited by GPT models''} (TF3) and that GPT-generated HWs tended to be \textit{``too generic (and) could be applied to anything''}. Student submissions exhibit creativity through diverse elements such as unique color selection, attractive animation effects, thoughtful variable naming, and a cohesive aesthetic.
    
    \item \textbf{GPT shows atypical usage of programming libraries [true].} TFs tended to believe the assignments were generated by GPT if they observed atypical usage of programming libraries. For example, TF2 successfully identified a GPT-generated HW, because \textit{``the mix of D3 and vanilla js in the main.js is somewhat odd''}.
    
    \item \textbf{GPT fails to read the visualization accurately [true].} TFs were able to identify submissions generated by GPT due to the model's inability to accurately interpret the content depicted in visualizations. For instance, GPT-generated textual descriptions might inaccurately refer to bar charts, even when there are no bar charts present in the visualization. GPT also generated visualizations in which the content was improperly positioned, e.g., \textit{``the map is half off the screen''} (TF2). This limitation arises because the current GPT model lacks the capability to directly interpret images and must make inferences based on code or textual descriptions.

    % \item \textbf{GPT includes errors that are easy to fix [true].}    
    
    \item \textbf{GPT does not write informal content [false].} TFs generally held the belief that GPT does not produce informal or disorganized content. For example, TF1 commented \textit{``some comments are informal enough that they seem student written''}. As a result, they mistakenly categorized some submissions as \textit{``maybe human''} when evaluating them. 
\end{itemize}

It is noteworthy that these observations should be interpreted with caution due to the limited sample size, the selection of only high-quality student assignments, and the minimal prompt engineering employed in utilizing GPTs.
% Specifically, TFs tended to believe the assignments were generated by GPT if it include 
% abnormal code structure (e.g., \textit{``The mix of D3 and vanilla js in the main is somewhat odd''} (TF2) ), 
% % 
% lack of creativity () , 
% % 
% fail to interpret the visualization correct (\textit{``''}), 
% % 
% obvious errors that are easy to fix (), 
% % 
% poor styling 

% Human:
% % 
% [actually wrong heuristics]
% informal/messy: \textit{``some comments informal enough that they seem student written''} (TF1)
% \textit{``code is messy enough to make it look human''} (TF1)
% \textit{``a little bit less structured, so I suspect it's a human''} (TF3)
% %
% %
% [correct heuristics]
% creativity: \textit{``this level of creativity is not done by  GPT ''} (TF3)

% [correct heuristics]
% good visual appearance: \textit{``Colors look unique''} (TF2)
% \textit{``Has aesthetic consistency. Really feels human''} (TF2)

\subsection{Final Project}
We explored GPT-4's capabilities in completing visualization projects
and summarize the experiments we conducted:
\cmo{need a conclusion and exempt here}
\qianwen{One general impression is that we need to say more than just "GPT can do it". Also, we should add more examples to make this section more interesting to read.}

\qianwen{I think we can remove this para if running out of space. First, it is less interesting. second, based on 3.2 final project, the step-by-step instruction is defined by us.}
\para{Planning the Projects.}
We input the final project requirements from CS171 to GPT-4 and asked it to propose a project plan.
It successfully generated a project plan with
basic info,
background and motivation,
related work,
and required dataset.
When we further asked GPT-4 how to finish this project plan, it responded with step-by-step guidelines, including
research and review related work,
data collection,
data cleanup,
data analysis and visualization,
interpretation and discussion,
documentation and presentation,
submission and evaluation.
This implies that GPT has the capability to propose project plans and generate actionable guidelines,
which can be used to inspire students or moderate teamwork.

\para{Data Collection and Cleanup.}
% GPT-4 can suggest where to collect relevant datasets and write code to do data cleanup. 
% To investigate this potential, 
% we asked GPT to provide guidance on 
% how to obtain data to finish the plan it proposed.
% GPT generated a response that included suggestions on 
% which websites to find the data and which specific datasets to download.
% After downloading the datasets, we also asked GPTs to write code to clean the datasets.
% GPTs successfully generated data cleanup code that could
% merge datasets, 
% % ensuring data compatibility and consistency,
% handle missing or inconsistent data,% by imputing, interpolating, or removing the affected data points,
% derive relevant metrics,
% and save the cleaned dataset into new files 
% % such as annual averages, percentiles, and trends 
% using Python libraries like pandas and numpy.
GPT-4 can assist with data collection and cleanup. It suggested websites and specific datasets to download. 
Additionally, GPT-4 successfully generated Python code (using libraries like pandas and numpy) to clean the datasets, merge them, handle missing or inconsistent data, derive metrics, and save the cleaned data into new files.

% We then evaluated the quality of the guidance provided by GPT by asking experts in the field to rate the suggestions on a scale from 1 to 5 based on their usefulness and relevance to the task. Our results showed that GPT was able to provide useful guidance for obtaining and cleaning data, with an average rating of 3.8 out of 5. This suggests that GPT has the potential to assist with the data preparation process for data visualization tasks.


\para{Designing Exploratory Visualizations based on Datasets and User Requirements.}
We tested GPT's capability of designing exploratory visualizations based on the provided data and user requirements.
We provided a toy dataset from the World Happiness Report 2020 and asked GPT-4 to create an interactive visualization that allows users
to browse, filter, and compare different data.
GPT-4 created an interactive scatterplot using D3.js (\cmo{a figure?}), 
which allows users to select the X and Y axes using dropdown menus.
When the user hovers over a data point, 
a tooltip displays the country, region, and the selected axes' values.
\qianwen{I vaguely remember that it is challenging to do multi-view visualizations. Might be interesting to discuss it here.}

\cmo{critize and improve the design}
GPT-4 can also improve the visualizations based on user feedback. For instance, when we expressed the need to examine specific countries more closely within a graph, GPT-4 implemented a zooming interaction.
% We further asked GPT-4 to add a feature that enables users to select a small area in the graph to take a closer look at some countries. GPT-4 subsequently added a zooming interaction to the chart.
\cmo{one sentence conclusion?}

% However, we also observed that GPT's ability to design effective visualizations depends on the quality and completeness of the input data, as well as the specificity of the user requirements. 
% We believe that GPT's ability to design visualizations can be further enhanced by incorporating more advanced data processing and visualization design techniques into its training data, as well as by developing more sophisticated prompts and input formats for users to provide guidance to the model. Overall, our findings suggest that GPT has the potential to be a valuable tool for data exploration and visualization design in a wide range of applications.

\para{Reading Visualizations in SVG and JS.}
While the GPT-4 model we used does not support images as input,
we found that it was capable of reading and interpreting visualizations in
SVG format.
We tested this by providing GPT with a set of scatter plots in SVG format
and asking it to describe its observations.
GPT-4 was able to correctly describe the chart type,
mark shapes (e.g., circle),
encodings (e.g., x- and y-axis, and color of the circles),
and the range of the axes. \qianwen{does this observation mean that GPT cannot read patterns, e.g., trending in a line chart?}
In addition to the SVG, we further provided GPT-4 with the Javascript code of the scatterplot and asked it to describe what kinds of interactions 
it can perform on the visualization.
It successfully identified the available interactions (i.e., switching which data attributes are mapped onto an axis through interacting with the drop-down menu and zooming in the scatter plot).

\para{Interacting with Visualizations through Dispatching JS Events.}
We also asked GPT to interact with the chart by dispatching Javascript events.
It successfully generated code to update axes by selecting the dropdown menu,
resetting the zoom, 
and mimicking a hover event to show the tooltip of a country.
This means that GPT can interact with visualizations by triggering corresponding events in the underlying JavaScript code. 
With the ability to interact with visualizations, GPT could potentially support a wider range of tasks that require user engagement and exploration of data. 


\para{Insight Discovery and Communication}
For insight discovery, we asked GPT-4 to generate some codes to interact with a chart and feed the resulting SVG file to it.
GPT-4 not only can read insights from visualizations, but also contextualize these insights with its extensive background knowledge, and select relevant insights and modified tone based on the target audience.
For example, it identified that Gabon ``\emph{has a relatively high Logged GDP per capital value but a lower Healthy life expectancy compared to other countries with similar GDP per capital values}'' from the visualization.
It further explained this insight by that  Gabon is a country known for its rich natural resources, particularly oil and timber, but has limited access to healthcare.
GPT also tailored textual descriptions for varied audiences, including African governments, the UN, and primary school students.
% \para{Interacting with Visualizations to Discover Insights.}
% Next, we asked GPT-4 to interact with the chart to discover data insights.
% In the prompt, we told GPT-4 that we would run its generated code
% and feed the resulting SVG back into GPT, for it to discover the insights.
% GPT-4 generated some code to interact with the chart
% and asked us to report the result for it.
% After running the code, we provided the resulting SVG for GPT-4.
% It successfully observed the correlation, trend, clusters,
% and outliers from the scatter plot.
% For example, it identified that Gabon ``\emph{has a relatively high Logged GDP per capita value but a lower Healthy life expectancy compared to other countries with similar GDP per capita values.}''
% Furthermore, with rich background knowledge,
% GPT-4 could further explain the insights by
% stating that Gabon is a country known for its rich natural resources, particularly oil and timber but has
% limited access to healthcare,
% high prevalence of infectious diseases,
% insufficient public health spending,
% and inadequate infrastructure.
% This suggests that GPTs can be used in a wide range of applications
% such as \cmo{xx}, \cmo{xx}, and \cmo{xx}.

% \para{Presenting Data Insights for Different Targeted Users.}
% We provided a set of scatterplots in SVG format for GPT-4 and asked it
% to write textual reports for the government of African developing countries, the UN, and primary school students, respectively.
% GPT-4 was able to select the relevant insights from the charts
% and reported them in a tone fit for the target readers.

\para{Data Storytelling.}
% Finally, we provided GPT-4 with the raw dataset and a list of textual insights
% and asked it to create narrative visualizations to explain them.
% GPT used Python libraries to create a series of annotated scatter plots
% to present the insights.
% When we complained that these charts were too boring and we preferred scrolly-telling, GPT then generated an HTML-based scrolly-telling visualization by using D3.js and 
% Scrollama~\cite{}.
% We also tried to ask GPT-4 to create data movies to present the insights.
% However, it could only generate an outline of the video or a code boilerplate in Python to create the video.
% Just like GPT said, ``\emph{while it's not possible to create a full data video directly within this text response,}'', it can ``\emph{can guide you through the process of creating one.}''
GPT-4 is capable of generating narrative visualizations when provided with a dataset and a list of insights. By default, GPT-4 may opt for Python libraries and annotated scatter plots to create these visualizations. However, when specifically requested to implement scrolly-telling, GPT-4 can generate an HTML-based scrolly-telling visualization using D3.js and Scrollama.
Other more complicated narrative formats, such data movies, present a challenge for end-to-end generation.
However, GPT acknowledges this limitation and offers an alternative solution, responding ``\emph{while it's not possible to create a full data video directly within this text response ... (I) can guide you through the process of creating one.}''


==> tex/_deprecated/5-discussion_v1.tex <==
\section{Discussion and Conclusion}
Due to page limitations, we cannot fully expand our discussion here. 
We briefly outline the key points that warrant future research. % in the future

\para{Facilitating Broader Visualization Tasks with LLMs.}
Our experiments demonstrate the potential of LLMs in facilitating broader visualization tasks. 
Through our investigation, 
we found that GPTs have rich knowledge of visualization design,
and can be utilized to design exploratory visualizations, read visualizations in SVG format, interact with visualizations through dispatching JavaScript events, and even create fancy narrative visualizations for general audiences. 
These findings highlight the vast capabilities of LLMs and their potential to complete or automate complex visualization tasks. 
In this sense, LLMs can be viewed as ``visualization experts'' that can provide valuable assistance to novices in visual data tasks. 
The potential of LLMs to enhance a broad range of visualization tasks for individuals with varying levels of expertise presents exciting opportunities for future research.



\qianwen{I feel we do need to discuss the limitation of GPTs in the discussion. Maybe a short discussion about, among all different visualization tasks, which are easier and which are more challenging. for example, good at communicating insights because it can adjust based on audience and contextualize it with background knowledge. not good at complicated narrative visualizations such as data videos. not good at multi-view visualizations (?).}

% Moreover, our results suggest that LLMs can serve as valuable tools in the visualization community, facilitating the development of innovative and effective visualization solutions. 

% in this area could explore how LLMs can be utilized to augment human intelligence and enable novel approaches to data visualization.

\para{Redesigning Visualization Education}
is an important task for the community.
Our experiments show 
that students in a visualization class can easily score well without truly learning the covered material. 
This highlights the need to rethink and redesign the way we teach visualization. 
One approach is to include tasks that are hard or impossible for GPTs to perform well alone. 
For instance, we could consider removing multiple-choice and single-choice questions and including more open-ended questions that involve skills such as sketching or rely on unique information/data provided in the class.
Another solution is to incorporate more group projects that promote teamwork and collaboration. \cmo{cite the design sprint paper?}
% In-class activities, such as discussions and debates, can also enhance students' learning experience. 
On the other hand, we can think about how GPTs can enhance human agency in the learning process. 
% Additionally, we can explore ways to 
For example, GPTs can be more creative with proper prompts from the students. %, providing a collaborative and personalized approach to learning; 
Teaching students how to use GPTs to solve visualization problems could provide a human/AI collaborative and personalized approach to learning.
Overall, it is essential to redesign visualization courses to better evaluate students' learning and promote their engagement with the material.

%- include more tasks that are hard or impossible for GPTs to perform well alone:  Should we remove multi-choice and single-choice questions since GPTs can easily answer them.
%Group projects that require teamwork
%In class activities

%- Enhancing human agency: some examples for good human-AI collaboration includes: GPT can be more creative with proper prompts from the students


\para{Limitations.} \jb{this should not be the last section of the paper!}
We acknowledge several limitations in our work. 
First, our sample size is limited to only a single offering of the CS171 course at Harvard University and the feedback from only three TFs. 
This may not be representative of other institutions or courses. 
Second, we only used high-quality student assignments for our comparison with GPTs, which may not reflect the overall performance of students in the course. 
Third, the minimal prompt engineering employed in utilizing GPTs may have constrained their performance, and more sophisticated prompts could lead to better results. 
Lastly, our findings may only apply to the two specific GPT models we used, and other models may have different capabilities and limitations. Further research is needed to address these limitations and explore the generalizability of our results.

% - limited sample size, 
% - the selection of only high-
% quality student assignments, 
% - the minimal prompt engineering employed in utilizing GPTs
% - only applies to the specific two GPT models wer are using
